LeanTutor: Towards a Verified AI Mathematical Proof Tutor

This paper considers the development of an AI-based provably-correct mathematical proof tutor. While Large Language Models (LLMs) allow seamless communication in natural language, they are error prone. Theorem provers such as Lean allow for provable-correctness, but these are hard for students to learn. We present a proof-of-concept system (LeanTutor) by combining the complementary strengths of LLMs and theorem provers. LeanTutor is composed of three modules: (i) an autoformalizer/proof-checker, (ii) a next-step generator, and (iii) a natural language feedback generator. To evaluate the system, we introduce PeanoBench, a dataset of 371 Peano Arithmetic proofs in human-written natural language and formal language, derived from the Natural Numbers Game.

==> Sections/desiderata.tex <==
\label{sec:desiderata}
What do we desire from a ``perfect'' math proof tutor?% that builds on LLMs, theorem provers and ITS? 
We are inspired by the design principles for general interactive tutoring systems~\cite{corbett1997intelligent}, \citet{molich1990improving} interface design principles, and the learner-centered design criteria proposed by \citet{keenanlearner} for classroom proof assistants. %We also consider the advantages and limitations of LLMs and theorem provers. 






Minimally, on the student interaction side, we would want the system to be \textbf{provably-correct}, \textbf{interact in natural language}, and \textbf{provide student-centric feedback}, i.e. follow the student line-of-thought on a proof. 
%
On the deployment side, we would need the system to be \textbf{scalable} to thousands of students, \textbf{instructor-adaptable} and \textbf{easy-to-deploy}, otherwise it will not be adopted. These minimal desiderata create a new set of research challenges, and we explore one approach to them here. 

%\subsubsection{Student-tutor interaction criteria} Minimally, we want the prover to: be \textit{provably-correct}, \textit{interact in natural language}, and \textit{provide student-centered feedback}. We aim to leverage LLMs' ability to broadly converse in natural language in tutoring applications. Conversely, requiring controlled natural language or a formal syntax is a key reason theorem provers have not seen greater use in classrooms \citep{karsten2023proofbuddy, thoma2022learning}. However, introducing an LLM into a tutor introduces stochastic slack into the system. An external verifier, such as a theorem prover, should be in place to validate LLM responses. Finally, tutor feedback should directly follow from the student's input---not regurgitate the staff solution or generate an entirely new solution.  

%\subsubsection{Deployment-based criteria} To encourage adoption of this math tutor, it should also be \textit{scalable} to large class sizes, \textit{instructor-adaptable}, and \textit{easy-to-deploy}. We should be able to robustly deploy a scalable tutor in a large university classroom, with minimal support or intervention from course staff. There should be minimal friction when adapting this tutor in any math course, or incorporating new material into an existing tutor. This math tutor should also adapt to the instructor's norms (i.e. notation, terminology) and curriculum (the tutor should not draw upon advanced material to demonstrate simpler concepts). 

\subsubsection{Resulting Design Challenges} In this work, we build towards a math tutor that fulfills the above criteria, by verifying an LLM tutor's outputs with the Lean theorem prover. This compound system requires a seamless back-and-forth between the LLM and theorem prover by means of faithful auto-formalization and auto-informalization. 

This requirement introduces new research challenges in the AI for Math field. It is already a technically challenging machine learning problem to train a capable formalization model, but fundamental differences between informal and formal math further complicate this task. 

These include a difference in granularity, as formal math proofs are much more fine-grained than informal ones, and a difference in reasoning paths, with informal proofs commonly written in a forward reasoning manner and formal ones in a backwards manner. Another key challenge in training this model is in accurately measuring the faithful autoformalization of correct and incorrect student proofs. No such metric currently exists to measure the faithful autoformalization of incorrect proofs. \textit{Pass@k} is a common metric used to measure model performance in successfully generating code or theorems \citep{chen2021evaluating, lisurvey}. This metric does not apply in the tutoring setting, since generations must be correct on the first pass. 

LeanTutor simplifies some of these challenges through a carefully aligned informal-formal math dataset, discussed in \ref{sec:peanobench}, and proposing a new ``relaxed exact matching metric'' to measure autoformalization accuracy (explained in \ref{sec:ourmetrics}), but by no means solves them. These design challenges remain as open research questions for the AI for Math and AI for Education communities. 

%So what do we desire from a ``perfect'' math proof tutor? Due to space limitations, we further discuss these in the paper appendix~\ref{sec:desiderata}.
